Operator Inference and Physics-Informed Learning of Low-Dimensional Models for Incompressible Flows

Reduced-order modeling has a long tradition in computational fluid dynamics. The ever-increasing significance of data for the synthesis of low-order models is well reflected in the recent successes of data-driven approaches such as Dynamic Mode Decomposition and Operator Inference. With this work, we suggest a new approach to learning structured low-order models for incompressible flow from data that can be used for engineering studies such as control, optimization, and simulation. To that end, we utilize the intrinsic structure of the Navier-Stokes equations for incompressible flows and show that learning dynamics of the velocity and pressure can be decoupled, thus leading to an efficient operator inference approach for learning the underlying dynamics of incompressible flows. Furthermore, we show the operator inference performance in learning low-order models using two benchmark problems and compare with an intrusive method, namely proper orthogonal decomposition, and other data-driven approaches.

==> sec-innerproduct.tex <==
\section{Inner product replaced}
\subsection{Petrov-Galerkin projection based model reduction of DAE systems}
In order to preserve the DAE structure, one could consider block Galerkin projections. Hence, one aims at finding projection matrices $\bV_v, \bW_{v}\in \R^{n_v \times r_v}$ and $\bV_p\in \R^{n_p \times r_p}$, with $\bW_v^T\bE_{11}\bV_v = \bI_{r_v}$.
Therefore, this leads to the reduced order model preserving the DAE structure 
\begin{subequations}
	\begin{align}
	\bhE_{11}\dbhv(t) &= \bhA_{11}\bhv(t) + \bhA_{12}\bhp(t) + \bhH\left(\bhv \otimes \bhv\right)  + \bhB_1 +\bhB_2 \bu(t)  ,  \\ 
	0 &=  \bhA_{12}^T\bv(t),  
	\end{align}
\end{subequations}
where
\begin{align*}
\bhE_{11} = \bW_v^T\bE_{11}\bV_v = \bI_{r_v}, \quad \bhA_{11} = \bW^T_v\bA_{11}\bV_v, \quad \bhA_{12} = \bW_v^T\bA_{12}\bV_p,\\  
\bhH = \bW_v^T\bH\left(\bV_v \otimes \bV_v\right), \quad  \bhB_1 =\bW_v^T\bB_1 \quad \text{and}  \quad \bhB_2 =\bW_v^T\bB_2
\end{align*}
The above projected system is obtained by a Galerkin block projection to the linear part using
\[\bV = \begin{bmatrix}
\bV_v & \\
& \bV_p
\end{bmatrix} \quad \text{and} \quad \bW = \begin{bmatrix}
\bW_v & \\
& \bV_p
\end{bmatrix} \]
and adapting the nonlinear part accordingly.
\subsection{Projected trajectories in this framework}
Let $0 = t_0 < t_1 < \dots <t_N = T$ be a time discretization of the interval $[0, T]$. Hence, we can define the trajectory, obtained by numerical solution of the the DAE \eqref{eq:DisctNavSto}, as 
\[\bV = \begin{bmatrix}
\bv(t_0) & \bv(t_1) & \dots & \bv(t_N)
\end{bmatrix}\quad \text{and} \quad \bP = \begin{bmatrix}
\bp(t_0) & \bp(t_1) & \dots & \bp(t_N)
\end{bmatrix} \]
with the corresponding input matrix 
\[\bU = \begin{bmatrix}
\bu(t_0) & \bu(t_1) & \dots & \bu(t_N)
\end{bmatrix}, \]
and mass times velocity derivatives 
\[\bE_{11}\dbV =\begin{bmatrix}
\bE_{11}\dbv(t_0) & \bE_{11}\dbv(t_1) & \dots & \bE_{11}\dbv(t_N)
\end{bmatrix}.  \]
  
 Instead of considering  the POD basis vectors from the SVD of $\bV\bV^T$, one can use the basis coming from the following SVD:
\begin{equation}
\bV\bE_{11}\dbV^T  \approx \bV_v \boldsymbol{\Sigma} \bW_{v}^T
\end{equation}
This SVD will lead to two POD basis, $\bV_v$ which gives information for the velocity subspaces, and  $\bW_{\bM}$ which gives information about the subspaces from mass times the velocity derivatives. As a consequence, we can use this two subspaces to get the information about the projected trajectories 
\[\bhV = \begin{bmatrix}
\bhv(t_0) & \bhv(t_1) & \dots & \bhv(t_N)
\end{bmatrix}  = \bV_v^T\bV \quad \text{and} \quad \dbhV =\begin{bmatrix}
\dbhv(t_0) & \dbhv(t_1) & \dots & \dbhv(t_N)
\end{bmatrix} = \bW_{v}^T\bE_{11}\dbV. \]
Also, let $\bV_p$ be the POD basis for the velocity. Then the projected velocity trajectories are given by:
\[\bhP = \begin{bmatrix}
\bhp(t_0) & \bhp(t_1) & \dots & \bhp(t_N)
\end{bmatrix} = \bV_p^T\bP   \]

\newpage
\section{Standard operator inference and Navier-Stokes model}

After discretization, one obtains a system of differential algebraic equations (DAE) of the form:
\begin{subequations}\label{eq:DisctNavSto}
	\begin{align}
	\bE_{11}\dot{\bv}(t) &= \bA_{11}\bv(t) + \bA_{12}\bp(t) + \bH\left(\bv \otimes \bv\right)  +  \mathbf{f}_1(t), \label{eq:DiffEq} \\ 
	0 &=  \bA_{21}\bv(t) + \mathbf{f}_2(t), \label{eq:AlgEq}  
	\end{align}
\end{subequations}
where $\bv(t) \in \R^{n_v}$, $\bp(t) \in \R^{n_p}$ are, respectively , the velocity and the pressure,  with $n_v>n_p$,  and  $\bE_{11}, \bA_{11} \in \R^{n_v \times n_v}$, $\bA_{12}^T, \bA_{21} \in \R^{n_p \times n_v}$, $\mathbf{f}_1(t) \in \R^{n_v \times 1}$, $\mathbf{f}_2(t)\in \R^{n_2\times 1}$. Furthermore, we assume that $\bE_{11}$ and $\bA_{21}\bE_{11}^{-1}\bA_{12}$ are nonsingular matrices. Additionally, we will suppose that the forcing terms are giving by
\begin{equation}
\mathbf{f}_1(t) = \bB_1 +\bB_2 \bu(t) \quad \text{and} \quad \mathbf{f}_2(t) \equiv 0,
\end{equation} 
where $u(t)\in \R^m$ are the inputs, with $\bB_1 \in \R^{n_v \times 1}$, $\bB_2 \in \R^{n_v \times m}$.

\section{Projection based model reduction of DAE systems}
In order to preserve the DAE structure, one could consider block Galerkin projections. Hence, one aims at finding projection matrices $\bV_v\in \R^{n_v \times r_v}$ and $\bV_p\in \R^{n_p \times r_p}$, with $\bV_v^T\bE_{11}\bV_v = \bI_{r_v}$,  such that, 
\[\bv(t) \approx \bV_v \bhv(t) \quad \text{and} \quad \bp \approx \bV_p \bhp(t). \] 
Therefore, this leads to the reduced order model preserving the DAE structure 
\begin{subequations}\label{eq:ROMNavSto}
	\begin{align}
	\bhE_{11}\dbhv(t) &= \bhA_{11}\bhv(t) + \bhA_{12}\bhp(t) + \bhH\left(\bhv \otimes \bhv\right)  + \bhB_1 +\bhB_2 \bu(t)  , \label{eq:Red_DiffEq} \\ 
	0 &=  \bhA_{12}^T\bv(t), \label{eq:Red_AlgEq}  
	\end{align}
\end{subequations}
where
\begin{align*}
\bhE_{11} = \bV_v^T\bE_{11}\bV_v = \bI_{r_v}, \quad \bhA_{11} = \bV^T_v\bA_{11}\bV_v, \quad \bhA_{12} = \bV_v^T\bA_{12}\bV_p,\\  
\bhH = \bV_v^T\bH\left(\bV_v \otimes \bV_v\right), \quad  \bhB_1 =\bV_v^T\bB_1 \quad \text{and}  \quad \bhB_2 =\bV_v^T\bB_2
\end{align*}
The above projected system is obtained by a Galerkin block projection to the linear part using
\[\bV = \begin{bmatrix}
\bV_v & \\
& \bV_p
\end{bmatrix} \]
and adapting the nonlinear part accordingly. Notice that by construction, the velocity basis $\bV_v$  satisfies the algebraic constrains, i.e., 
\[ 0 =  \bhA_{12}^T\bV_v.\] 
As a consequence,
\[ \bhA_{12} = \bV_v^T\bA_{12}\bV_p = 0, \]
and the reduced POD model is pressure independent and has the above structure
\begin{subequations}\label{eq:ROMNavSto_quad}
	\begin{align}
	\dbhv(t) &= \bhA_{11}\bhv(t) + \bhH\left(\bhv \otimes \bhv\right)  + \bhB_1 +\bhB_2 \bu(t)  , \label{eq:Red_DiffEq_quad}
	\end{align}
\end{subequations}
and the algebraic constrains are automatically satisfied. 

Additionally, in order to obtain the pressure evolution, let us write
\[0  = \bA_{12}^T\bv (t). \]
By taking the derivative, one obtains
\[0  = \bA_{12}^T\dbv (t) =  \bA_{12}^T\bE_{11}^{-1}\bA_{11}\bv(t) + \bA_{12}^T\bE_{11}^{-1}\bA_{12}\bp(t) + \bA_{12}^T\bE_{11}^{-1}\bH\left(\bv \otimes \bv\right)  +  \bA_{12}^T\bE_{11}^{-1}\mathbf{f}_1(t). \]
As a consequence,
\[\bp(t) = -\Pi \bA_{11}\bv(t) -\Pi\bH\left(\bv \otimes \bv\right)  -\Pi \mathbf{f}_1(t).  \] 
where 
\[\Pi =  (\bA_{12}^T\bE_{11}^{-1}\bA_{12})^{-1}\bA_{12}^T\bE_{11}^{-1} \]

\subsection{Operator inference for Navier Stokes}

Let $0 = t_0 < t_1 < \dots <t_N = T$ be a time discretization of the interval $[0, T]$. Hence, we can define the trajectory, obtained by numerical solution of the the DAE \eqref{eq:DisctNavSto}, as 
\[\bV = \begin{bmatrix}
\bv(t_0) & \bv(t_1) & \dots & \bv(t_N)
\end{bmatrix}\quad \text{and} \]
with the corresponding input matrix 
\[\bU = \begin{bmatrix}
\bu(t_0) & \bu(t_1) & \dots & \bu(t_N)
\end{bmatrix}, \]
and velocity derivatives 
\[\dbV =\begin{bmatrix}
\dbv(t_0) & \dbv(t_1) & \dots & \dbv(t_N)
\end{bmatrix}.  \]
We suppose we have access to the above data from a black box simulator, but that the original realization from the system \eqref{eq:DisctNavSto} is not available. Let $\bV_v$ be the POD basis vectors. As a consequence we can also define the projected trajectory as
\[\bhV = \begin{bmatrix}
\bhv(t_0) & \bhv(t_1) & \dots & \bhv(t_N)
\end{bmatrix}  = \bV_v^T\bV \quad \text{and}  \]
with the projected velocity derivatives 
\[\dbhV =\begin{bmatrix}
\dbhv(t_0) & \dbhv(t_1) & \dots & \dbhv(t_N)
\end{bmatrix} = \bV_v^T\dbV.  \]

Our main goal is to be able to construct a reduced order model for  \eqref{eq:DisctNavSto} in a non-intrusive way. To this aim, let us write the reduced order model in \eqref{eq:ROMNavSto} as follows:
\begin{align}
\begin{bmatrix}
\bhA_{11}  & \bhH & \bhB_1 & \bhB_2 
\end{bmatrix} \begin{bmatrix}
\bhv(t) \\ 
\bhv(t) \otimes \bhv(t) \\
\mathbf{1}\\
\bu(t)
\end{bmatrix} = \begin{bmatrix}
\dbhv(t) 
\end{bmatrix}
\end{align}

Hence a first trial to obtain the reduced order model from the data would be to consider the following structured least squares problem:
\begin{prob}[\bf  least square problem] Find $\bhA_{11},  \bhH,  \bhB_1$ and  $\bhB_2$ such that
	\begin{equation}
	\min\limits_{\bhA_{11}, \bhA_{12}, \bhH , \bhB_1,\bhB_2} \left\| \begin{bmatrix}
	\bhA_{11} & \bhA_{12} & \bhH & \bhB_1 & \bhB_2 
	\end{bmatrix}\bhX -\bhD  \right\|^2_{F}
	\end{equation}
\end{prob}

\subsection{Navier Stokes with forcing algebraic term}

Now let us consider the general problem with algebraic forcing term:
\begin{subequations}\label{eq:DisctNavSto}
	\begin{align}
	\dot{\bv}(t) &= \bA_{11}\bv(t) + \bA_{12}\bp(t) + \bH\left(\bv \otimes \bv\right)  + \bB_1, \label{eq:DiffEq} \\ 
	0 &=  \bA_{12}^T\bv(t) + \bB_2, \label{eq:AlgEq}  
	\end{align}
\end{subequations}
Let us consider the following change of basis
\[ \bv_s(t) = \bv(t) + \bQ, \quad \text{with} ~\, \bQ = \bA_{12}(\bA_{12}^T\bA_{12})^{-1}\bB_2. \]
As a consequence, the system in this new variable is 
\begin{subequations}\label{eq:DisctNavSto}
	\begin{align}
	\dot{\bv}_s(t) &= \bA_{11}\bv_s(t) + \bA_{12}\bp(t) + \bH\left(\bv_s \otimes \bv_s\right)  + \btB_1, \label{eq:DiffEq} \\ 
	0 &=  \bA_{12}^T\bv_s(t) , \label{eq:AlgEq}  
	\end{align}
\end{subequations}
with 
\[  \btB_1 = \bB_1 -\bA_{11}\bQ\bB_2 - \bH(\bQ\bB_2\otimes\bQ\bB_2)  \]
Hence if one is able to compute $\bQ$ from the data, by transforming the data as above this problem ends up to be the same as the one without the forcing term. The questions is how to obtain this transformation from the snapshots.

\subsection{Data-driven transformation}
Notice that for any $\bT$ nonsingular matrix,  if $\bT\bA_{12}^T = \btA_{12}^T$ and $\bT\bB_{2} = \btB_{2}$, then
\[ \btA_{12}(\btA_{12}^T\btA_{12})^{-1}\btB_2 = \bA_{12}\bT^T(\bT^T\bA_{12}^T\btA_{12}\bT^T)^{-1}\bT\bB_2 = \bA_{12}(\bA_{12}^T\bA_{12})^{-1}\bB_2 = \bQ  \]

Hence, one can get the matrices $\bT \bA_{12}^{T}$ and $\bT\bB_2$ as being one of the left kernel solution of 
\[ \begin{bmatrix}
\bX_1 & \bX_2
\end{bmatrix} \begin{bmatrix}
\bV \\ 
\bU
\end{bmatrix} = 0  \]


==> sec-lit-overview.tex <==

\subsection{Literature overview}
The numerical solution of the incompressible Navier-Stokes equation is a
demanding task in terms of computational effort and memory requirements. 
Reduced order models can significantly decrease the demands while maintaining a
certain accuracy. One may well say, that flow simulations have been a success
story for the application of model reduction schemes as well as a driving force
for the development of new approaches. For example, the popular methods of
\emph{Proper Orthogonal Decomposition} and \emph{Dynamic Mode Decomposition}
seem to have their origins in flow computations; see \cite{morSir87a,morSch10}. On
the other hand the distinguished nonlinear and differential-algebraic structure
of the semi-discrete incompressible Navier-Stokes has been attractive for the
testing of extensions of standard system-theoretic approaches like LQGBT,
moment-matching, or polynomial expansions of the HJB equations; see
\cite{morAhmBGetal17,morBenH15,BreKP19}.

POD in flows -- see the refs in \cite{morGraHLU19} + a look at Carlberg.

This manuscript introduces the method of \emph{Operator Inference} for the
incompressible Navier-Stokes equation. 

While for POD the actual model is needed, for OPINF only assumptions on the
structure of the model are made.



